Streaming Verification of Graph Properties

Streaming interactive proofs (SIPs) are a framework for outsourced computation. A computationally limited streaming client (the verifier) hands over a large data set to an untrusted server (the prover) in the cloud and the two parties run a protocol to confirm the correctness of result with high probability. SIPs are particularly interesting for problems that are hard to solve (or even approximate) well in a streaming setting. The most notable of these problems is finding maximum matchings, which has received intense interest in recent years but has strong lower bounds even for constant factor approximations. In this paper, we present efficient streaming interactive proofs that can verify maximum matchings exactly. Our results cover all flavors of matchings (bipartite/non-bipartite and weighted). In addition, we also present streaming verifiers for approximate metric TSP. In particular, these are the first efficient results for weighted matchings and for metric TSP in any streaming verification model.

==> mcmb.tex <==
\section{SIP for MAX-MATCHING in Bipartite Graphs}
\label{sec:mcmb}
We now  present a SIP for maximum cardinality matching in bipartite graphs. The prover \textsf{P} needs to generate two certificates: an actual matching, and a proof that this is optimal. By K\"{o}nig's theorem \cite{konig}, a bipartite graph has a maximum matching of size  $k$ if and only if it has a minimum vertex cover of size $k$. Therefore, \textsf{P}'s proof consists of two parts:
\begin{inparaenum}[a)]
  \item Send the claimed optimal matching $M\subset E$ of size $k$
  \item Send a vertex cover $S\subset V$of size $k$. 
\end{inparaenum}
\textsf{V} has three tasks:
\begin{inparaenum}[i)]
  \item Verify that $M$ is a matching and that $M \subset E$.
  \item Verify that $S$ covers all edges in $E$. 
  \item Verify that $|M| = |S|$.
\end{inparaenum} We describe protocols for first two tasks: the third task is trivially solvable by counting the length of the streams and can be done in $\log n$ space. \textsf{V} will run the three protocols in parallel.\\\\
%\vspace*{-3mm}
\noindent\textbf{Verifying a Matching.}
%\vspace*{-2mm}
\label{sec:verifying-matching}
Verifying that $M \subset E$ can be done by running the \subgraph protocol from Lemma~\ref{lem:subgraph} on $E$ and the claimed matching $M$. A set of edges $M$ is a matching if each vertex has degree at most $1$ on the subgraph defined by $M$. Interpreted another way, let $\tau_M$ be the stream of endpoints of edges in $M$. Then each item in $\tau_M$ must have frequency $1$. This motivates the following protocol, based on Theorem \ref{thm:multi-set-equality}. \textsf{V} treats $\tau_M$ as a sequence of updates to a frequency vector $\mathbf{a} \in \integers^{|V|}$ counting the number of occurrences of each vertex. \textsf{V} then asks \textsf{P} to send a stream of all the vertices incident on edges of $M$ as updates to a different frequency vector $\mathbf{a}'$. \textsf{V} then runs the \mse protocol to verify that these are the same. \\\\
%\vspace*{-3mm}
\noindent\textbf{Verifying that $S$ is a Vertex Cover.}
%\vspace*{-2mm}
The difficulty with verifying a vertex cover is that \textsf{V} no longer has streaming access to $E$. However, we can once again reformulate the verification in terms of frequency vectors. $S$ is a vertex cover if and only if each edge of $E$ is incident to some vertex in $S$. Let $\mathbf{a}, \mathbf{a}' \in \integers^{\binom{n}{2}}$ be  vectors  indexed by $\mathcal{U} = \{(i,j), i, j \in V, i  < j\}$. On receiving the input stream edge $e = (i,j, \Delta), i < j$, \textsf{V} increments $\mathbf{a}[(i,j)]$ by $\Delta$.

For each vertex $i \in S$ that \textsf{P} sends, we increment all entries $\mathbf{a}'[(i, *)]$ and $\mathbf{a}'[(*, i)]$. Now it is easy to see that $S$ is a vertex cover if and only there are no entries in $\mathbf{a - a'}$ with value $1$ (because these entries correspond to edges that have \emph{not} been covered by a vertex in $S$). This yields the following verification protocol. 
\begin{enumerate}
\item \textsf{V} processes the input edge stream for the $F^{-1}_{1}$ protocol, maintaining updates to a vector $\mathbf{a}$. 
\item \textsf{P} sends over a claimed vertex cover $S$ of size $c^*$ one vertex at a time.  For each vertex $i \in S$, \textsf{V} \emph{decrements} all entries $\mathbf{a}[(i, *)]$ and $\mathbf{a}[(*, i)]$ 
\item \textsf{V} runs \finv to verify that $F^{-1}_1(\mathbf{a}) = 0$. 
\end{enumerate}

The bounds for this protocol follow from Lemmas \ref{lemma:finv}, \ref{lem:subgraph} and Theorem \ref{thm:multi-set-equality}: %Adding the communication and space bounds, we get the following result.
\begin{theorem}
Given an input bipartite graph with $n$ vertices, there exists a streaming interactive protocol  for verifying the maximum-matching with $\log n$ rounds of communication, and cost $(\log^2 n,   (c^* + \log n) \log n)$, where $c^*$ is the size of the optimal matching.
\end{theorem}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "verify_matchings"
%%% End:


==> mcmg.tex <==
\section{Streaming Interactive Proof for Maximum-Matching in general graphs}
\label{sec:mcmg}
The SIP protocol for verifying the maximum matching in general graphs consists of two parts as well: checking lower bound and upper bound for optimal matching.
\paragraph{The Lower bound Protocol}
As we know any feasible matching presents a lower bound, thus the protocol for checking lower bound for maximum matching in general case is the same as the one described before for bipartite case and here we ignore to repeat it again. 

\paragraph{The Upper bound Protocol}
Based on Tutte-Berge formula, we know that the size of maximum matching in the graph is:
\begin{align*}
\frac{1}{2} min _{V_s \subseteq V} (|V_S| - odd(G - V_S) + |V|)
\end{align*}

So for any set of nodes $V_S$, the value $(|V_S| - odd(G - V_S) + |V|$ will be an upper bound on the size of the maximum matching and in fact there exists some subset $V_S$ for which this quantity equals the size of a maximum matching $M$. 

This implies that the elements in $(|V_S| - odd(G - V_S) + |V|)$ can be used as certificates provided by the prover so verifier can check the upper bound value on the maximum matching $M$. The main part of this certificate is the list of all the connected components in $G - V_S$. For simplicity, consider $V - V_S = U = (U_i \cup \cdots \cup U_r)$ as the $r$ connected components and $T = (T_i \cup \cdots \cup T_r)$ as $r$ spanning trees on $r$ corresponding connected components, provided by prover as the certificate. 

Now verifier needs to check if the upper bound certificate is valid by considering the following conditions:
\begin{enumerate}
\item All the spanning trees are disjoint, i.e. $T_i \cap T_j = \emptyset$ for all the pairs of trees in $T$.
\item Each spanning tree in $T = (T_1 \cup \cdots \cup T_r)$ is a subgraph of the input graph $G$. This may be handled by our SUBGGRAPH protocol described earlier.
\item Each component in $T = (T_1 \cup \cdots \cup T_r)$  is in fact a \emph{spanning tree}.
\item Each component in $T = (T_1 \cup \cdots \cup T_r)$ is in fact maximal, i.e. there is no edge between the components in original graph $G$.
\end{enumerate}

We assume that the certificate $T$ is sent by prover in streaming manner in the following format and both players agree on this at the start of the protocol:
\begin{align*} 
T: \{|T|, r, (T_1 , \cdots , T_r) \}
\end{align*}
For the representation of spanning trees, we consider a topological ordering on each tree $T_i$, starting from root node $f_i$, and each directed edge $(v_\ell, v_t)$ connects the parent node $v_\ell$ to the child node $v_t$:
\begin{align*}
T_i: \{f_i, \cup e (v_{out}, v_{in})\}
\end{align*}

Here we present the protocols for checking each of these conditions. The following DISJOINTEDNESS protocol will be called as a subroutine in our $r$-SPANNING TREE main protocol.

\paragraph{Protocol 2: DISJOINTEDNESS}
\begin{enumerate}
\item \textsf{P} sends over $r$ components of $T_i$ in $T$ in streaming manner . 
\item \textsf{P} ``replays" all the edges $T'$ in the tuple form $(e_{i,j}, \ell)$ for $i$, $j \in [n]$ and $\ell \in [r]$ denotes the component $e_{i,j}$ is assigned to. The edges in $T'$ are presented according to a canonical total ordering on the edge set, and hence $\textsf{V}$ can easily check that $T'$ has no repeated edge; i.e., the same edge presented in two distinct components.
\item Fingerprinting can then be used to confirm that $T' = \cup_i T_i$ with high probability, and hence that each edge occurs in at most one tree.
\item A similar procedure is run to ensure that no vertex is repeated in more than one $T_i$.
\end{enumerate}
 

\paragraph{Protocol 3: k-SPANNING TREE}
To check if each component in the claimed certificate $T$ by prover is in fact spanning tree, the verifier needs to check that each of $T_i$ is \emph{cycle-free} and also \emph{connected}. For this goal we present the following protocol:

\begin{enumerate}
\item \textsf{P} sends over the certificate $T: \{|T|, r, (T_1 , \cdots , T_r) \}$ in which each $T_i: \{i, \cup e (v_{out}, v_{in})\}$.
Consider the root of each $T_i$ to be represented by the edge $(\phi_i, v_{i})$ where $v_i$ is the root of $T_i$. 
\item \textsf{V} runs the DISJOINTEDNESS protocol to ensure that in the certificate $T: \{|T|, r, (T_1 , \cdots , T_r) \}$ all  $T_i$ and $T_j$ are edge and vertex disjoint for all $i \neq j$.
\item \textsf{V} has the prover again similarly replay $\cup_i T_i$ ordered by the label of the in-vertex of each edge to ensure that each vertex except the $\phi_i$ has exactly one incoming edge; i.e, that all $T_i$ are cycle free and connected.
\end{enumerate}


We need to check that there is no edge between sets $U_i$ and $U_j$ for $i \neq j$. We present two alternative protocols for this check, where the first has better communication and space complexity, whereas the second has better verifier update time.

\paragraph{Protocol 4 a: MAXIMALITY A}
Our first protocol is inspired by that for max-weight bipartite matching \ref{sec:maxWBipartite}.  We define an extended universe $U$ now of size $n^3$, $(e_{i,j}, k )$ where $k \in [n]$ represents the label of the component in the Tutte-Berge certificate. 

\begin{enumerate}
\item \textsf{V} initiates the $F^{-1}(-1)$ protocol on the input stream. Upon seeing any edge $e_{i,j}$, $\textsf{V}$ increments by $1$ all tuples containing $e_{i,j}$.
\item \textsf{P} sends the label of each vertex $(v_i, j)$ where $j \in [n]$ represents the label of the component in the Tutte-Berge certificate, and $j = n+1$ denotes that the vertex is in $G-  U$. (Note that the verifier can ensure this input is consistent with the $T = \cup_i T_i$ sent earlier by simply fingerprinting as described earlier).

\item \textsf{V} considers each vertex $v_i \in U_j$  for $j \neq n+1$ as a decrement update by $2$ on all 
on all $n$ possible tuples compatible with $v_i$  and component label $j$. This step can be assumed as continuing the process for $F^{-1}(-1)$ mentioned in the first step.

\item \textsf{V} considers each vertex $v_i \in U_{n+1}$ as a increment update by $2$ on all $n^2$  possible tuples of the universe compatible with $v_i$.

\item $F^{-1}(-1)$ corresponds to exactly the set of edges between two $U_i$ and $U_j$ for $i \neq j$. To see this, we enumerate the cases explicitly:
\begin{enumerate}
\item $\{-2, -3 \}$ are the possible values for an edge $(e_{a,b}, i)$ with both endpoints contained in a single $U_i$ corresponding to whether $e_{a,b}$ was originally in the stream or not. (The edge is decremented twice by $2$ in the derived stream.

\item $\{0,1 \}$ are the possible values for any edge $(e_{a,b}, i)$ with one endpoint in a $U_i$ and the other in $G-U$, corresponding to whether $e_{a,b}$ was originally in the stream or not. (The edge is incremented and decremented once each by $2$ in the derived stream.)

\item $\{4,5 \}$ are the possible values for any edge $(e_{a,b}, i)$ with both endpoints ina $G-U$, corresponding to whether $e_{a,b}$ was originally in the stream or not. (Each such edge is incremented twice each by $2$ in the derived stream.)

\item $\{-1,-2 \}$ are the possible values for any edge $(e_{a,b} , i)$ and $(e_{a,b} , j)$ with one endpoint in a $U_i$ and the other in $U_j$ for $i \neq j$, corresponding to whether $e_{a,b}$ was originally in the stream or not. (The edge is incremented and decremented exactly once by $2$ in the derived stream).
\end{enumerate}

\item \textsf{V} runs $F^{-1}$ with $\textsf{P}$ and accepts that there are no edges between the $U_i$ if and only if $F^{-1}(-1) = 0$.

\end{enumerate} 

\paragraph{Complexity Analysis of The Protocol}
We know the cost of $F^{-1}(5)$ protocol is $(\log n, \log n)$ for frequency ranges bounded by a constant, whereas the costs of the remaining fingerprinting steps and sending the certificate are at most  $(\log n, n \log n)$.  Hence the cost of our protocol is dominated by $(\log n, n \log n)$ in the worst case. The verifier update cost on each step is bounded as $O(n^2)$.

\paragraph{Protocol 4 b: MAXIMALITY B}
Our second  protocol is inspired by that for checking if a graph is bipartite (Section \ref{sec:check_bipartite}), particularly the sub-protocol for checking all edges cross a bipartition. As compared to Protocol 4 a, the advantage is that the verifier update time is less, although the protocol cost is slightly more.

First assume \textsf{V} has oracle access to a strictly monotone function $f_{A} : [r] \to [m]$, for a positive integer $m$ to be set later, such that:
\begin{itemize}
\item $f_{A}$  is 3-AP free, i.e., $f_{A}(a) + f_{A}(b) \neq 2 f_{A}(c)$ for any three distinct elements $a,b,c \in [k]$.
\item $f_{A}(i)$ mod $5 = 2$, $\forall i \in [r]$.
\end{itemize} 
Define $X_A = \{ x : x = 1-f_A(i) - f_A(j)$, $i \neq j$, $i$,$j \in [r]  \}$. Note that 
$|X_A| \leq 2m - 1$. 
\begin{enumerate}
\item \textsf{V} processes the input data stream for $F^{-1}(X_A)$ protocol (with respect to frequency vector $\mathbf{a}$ defined over all the possible edges in complete graph with $n$ vertices and stream updates as edges in input). 
\item \textsf{V} considers each vertex $v \in U_i$ as a decrement update by $f_i$ 
on all the possible incident edges to $v$ in complete graph over the frequency vector $\mathbf{a}$. This step can be assumed as continuing the process for $F^{-1}(X_A)$ mentioned in the first step.
\item At the end of this step, the possible values in vector $\mathbf{a}$ (depending on whether an edge was originally present in graph or not) will be:
\begin{enumerate}
\item $\{- 2 f_A(i) , 1 - 2 f_A(i) \}$ for all the possible edges $e: (v, v')$ in which both endpoints $v, v' \in U_i$. 
\item $\{ 0, 1 \}$ for edges in which both endpoints are in $V \setminus U$.
\item $\{- f_A(i), 1 - f_A(i)  \}$ for all the possible edges $e: (v, v')$ in which there is an endpoint in each of $U_i$ and $V \setminus U$ for some choice of $i \in [k]$.
\item $\{- f_A(i) - f_A(j), 1 - f_A(i) - f_A(j) \}$ for all the possible edges $e: (v_i, v_j)$ in which there is an endpoint in each of $U_i$ and $U_j$ for $i \neq j$.
\end{enumerate}
\item Note that the ``bad" cases are where an edge $e$ originally appeared in the input stream and has its endpoints in $U_i$ and $U_j$ for some $i \neq j$. After our stream of decrements, the frequency of such a bad edge $e$ corresponds to $1 - f_A(i) - f_A(j)$ for some choice of $i$, $j$, which is an element of $X_A$. As such, the verifier now runs the protocol to confirm $F^{-1}(X_A) = 0$. 
\end{enumerate}

We have to confirm though that there are no ``collisions" between $X_A$ and the values induced by the other possible cases which do not correspond to edges between $U_i$ and $U_j$ for $i \neq j$. 
We proceed by case-wise analysis. The following observation will be useful:

\begin{lemma} Every element of $X_A$ will be $2$ mod $5$.
\end{lemma}

\begin{proof}
$1 - 2 - 2 = -3 = 2$ mod $5$.
\end{proof}

\begin{enumerate}
\item Consider the case $\{- 2 f_A(i) , 1 - 2 f_A(i) \}$ for the possible edges $e: (v, v')$ in which both endpoints $v, v' \in U_i$ and some choice of $i$. Note that $- 2 f_A(i)$ is $1$ mod $5$, and hence cannot collide with $X_A$. 

Secondly, a collision of the $1 - 2 f_A(i)$ with $X_A$ would imply either that
\begin{enumerate} 
\item  $1 - 2 f_A(i) = 1 - f_A(j) - f_A(k)$, for distinct $i$,$j$, $k$. This then means $2 f_A(i) = f_A(j) + f_A(k)$ and hence contradicts our construction that $f$ is $3$-AP free.  
\item $1 - 2 f_A(i) = 1 - f_A(i) - f_A(j)$ for distinct $i$, $j$. This would imply that $f_A(i) = f_A(j)$ for $i \neq j$ which contradicts our construction that $f$ is strictly monotone.
\end{enumerate} 
\item For the case where both endpoints are in $G-U$, the possible range of frequencies is $\{0, 1 \}$ and hence may not collide with $X_A$ which is strictly negative.
\item Next consider $\{- f_A(i), 1 - f_A(i)  \}$ for all the possible edges $e: (v, v')$ in which there is an endpoint in each of $U_i$ and $V \setminus U$ for some choice of $i \in [k]$. Note that $-f_A(i)$ will be $-2 = 3$ mod $5$ and $1- f_A(i)$ will be $-1 = 4$ mod $5$ and hence cannot collide with $X_A$.
\item Finally, one can clearly see that $-f_A(i) - f_A(j)$ cannot collide with $X_A$ as 
$-f_A(i) - f_A(j) = 1$ mod 5.
\end{enumerate}

Note that given the existence of a function $f_{A} : [r] \to [m]$ which is only known to be $3$-AP free, we can derive a function $f'_{A} : [\lceil r/5 \rceil ] \to [m+5]$, such that $f'_{A}$ $3$-AP free as well as satisfying that $f_{A}(i) = 2$ mod $5$, $\forall i \in [r]$.  To see this, simply split the range of $f_{A}$ into the modulo classes $C_0$, $C_1$, $C_2$, $C_3$ and $C_4$ w.r.t. $5$. By the pigeonhole principle, there must be some $C_j$ of size at least $\lceil r/5 \rceil$. We can shift $C_j$ to be $2 \mod 5$ by adding $2-j$ to every element of $C_j$, and letting this $C_j$ be the range of $f'_{A}$. Observe also that adding a constant does not affect the $3$-AP free nature of $f'$.

\paragraph{Complexity Analysis of The Protocol}
We know the cost of $F^{-1}(X_A)$ protocol is $(\log n, |X_A| \log n)$, whereas the costs of the remaining fingerprinting steps and sending the certificate are at most  $(\log n, n \log n)$.   Since $|X_A|$ may in the worst case be superlinear in $n$, hence the cost of our protocol is dominated by $(\log n, |X_A| \log n)$. The verifier update cost on each step is bounded as $O(n)$. 

(Note that the verifier update cost on each step is less here,but the communication cost is slightly more.)


\paragraph{Protocol 5:  Generation of $f_A$}
As mentioned in the previous protocol the strictly monotone function $f_A: [r] \to [m]$ must have the following two properties,
\begin{itemize}
\item $f_A$ is $3$-AP free\\
Let's denote the range of $f_A$ by a set $S(d,k)$ for some fixed $d, k$. Elements of this set can be generated using the following formula \cite{pmid16588588}
\begin{align}
\label{eqn:g1}
A = a_1 + a_2(2d - 1) + a_3(2d - 1)^2 + \ldots + a_k(2d - 1)^{k-1}
\end{align}
where $d > 2, k|d, a_i \in [0\ldots d-1]$ and each $a_i$ occurs exactly $k/d$ times.

In \cite{pmid16588588} Salem and Spencer showed that, given a fixed maximum value of such a sequence (i.e. $m$), the length $l(m)$ of the sequence has the following lower bound $\forall \epsilon > 0$,
\begin{align}
\label{eqn:b1}
l(m) > m^{1 - \frac{\log 2 + \epsilon}{\log \log m}}
\end{align}
As mentioned before the complexity of the \emph{MAXIMALITY B} protocol is dominated by the complexity of $F^{-1}(X_A)$ which is $(\log n, |X_A|\log n)$, and we know $|X_A|\leq 2m - 1$. Now it can be shown that $m = O(|U|^{1 + \delta}) with l(m) > |U|$, where $\delta > \frac{a}{\log\log|U| - a}, \forall a > \log2$ . And as $|U| \leq n$, therefore the complexity is $(\log n, n^{1 + \delta}\log n)$.
This can be shown like the following by replacing $m$ in the RHS of the inequality \ref{eqn:b1},
\begin{align*}
|U|^{(1 + \delta)(1 - \frac{\log 2 + \epsilon}{\log (1 + \delta) + \log\log |U|})} &\geq |U|\\
(1 + \delta)(1 - \frac{\log 2 + \epsilon}{\log (1 + \delta) + \log\log |U|}) &\geq 1\\
1 - \frac{\log 2 + \epsilon}{\log (1 + \delta) + \log\log |U|} &\geq \frac{1}{1 + \delta}\\
1 - \frac{a}{\delta + \log\log|U|} &\geq \frac{1}{1 + \delta} \quad \textrm{As $\log(1 + \delta) \leq \delta$, and replacing $\log 2 + \epsilon = a$}\\
\delta^{2} + \delta(\log\log|U| - a) - a &\geq 0\\
\end{align*}
Solving for $\delta$ considering equality and ignoring the negative root\\
\begin{align}
\delta &= \frac{(a - \log\log|U|) +\sqrt{(\log\log|U| - a)^2 + 4a}}{2}\nonumber\\
\delta &> \frac{a}{\log\log|U| - a} \quad \textrm{Simplified by taking first 2 terms of bionomial expansion} \label{eqn:del}
\end{align}

\cdnote {Need to complete how to choose $d$ and $k$ using the inequality $(2d - 1)^{dg(d)} \leq m < (2d + 1)^{(d+1)g(d+1)}$.}

According to Salem and Spencer \cite{pmid16588588} the value of $d, k$ in equation \ref{eqn:g1} should be such that, the following inequalities are satisfied,
\begin{align}
(2d - 1)^{dg(d)} &\leq m < (2d + 1)^{(d+1)g(d+1)}\label{eqn:in1}
\end{align}
where $\lim_{d \to \infty}\frac{g(d)}{\log d} = \infty$ and $\lim_{d \to \infty}\frac{\log g(d)}{\log d} = 0$. This means that $g(d)$ is super linear in $\log d$ and $g(d) < d$, therefore we can assume $g(d) = \log^{t}d$ for $t > 1$.
By taking logarithms, we have the following two inequalities,
\begin{align}
\log m &\geq dg(d)\log (2d - 1) \label{eqn:l1}\\
\log\log m &< \log (d+1) + \log g(d+1) + \log \log (2d + 1)\label{eqn:u1}
\end{align}
Using the above inequalities \ref{eqn:l1}, \ref{eqn:u1} as shown by Salem and Spencer\cite{pmid16588588} we get
\begin{align*}
\frac{\log m}{\log\log m} &> \frac{dg(d)\log (2d - 1)}{\log (d+1) + \log g(d+1) + \log \log (2d + 1)}\\
\frac{\log m}{\log\log m} &> dg(d)[1 + o(1)]\\
\log m &> dg(d)\\
\log m &> d
\end{align*}
Thus we know $d$ is upper bounded by $\log m = (1 + \delta)\log |U|$. We can assume that the verifier gets appropriate $d, k$ from an external oracle given $m$ that satisfies the ineqaulity \ref{eqn:in1}.

The verifier can query the prover to get the number of connected components i.e. $|U|$. Now verifier gets suitable $d, k$ by fixing $m = (5|U|)^{1+\delta}$ for some $\delta$ satisfying the inequality \ref{eqn:del}. The verifier then generates $5|U|$ numbers in increasing order starting with the smallest lexicographic permutation 
\[ (a_k, a_{k-1}, \ldots , a_1) = (0 \ldots k/d \text{ times }, 1 \ldots k/d \text{ times }, \ldots , d-1 \ldots k/d \text{ times }) \] 
and calling \emph{next-permutation} $5|U|$ times generating numbers that are strictly larger than previously generated ones. The space to store this permutation is $O(k\log d) = O(\log\log^{t}|U|)$ for some constant $t$. \emph{next-permutation} has worst case complexity $O(k)$ as there are $k$ digits, and amortized $\mathcal{O}(1)$ cost if it is called $\frac{k!}{(\frac{k}{d}!)^d}$ time. With known $d, k$, the verifier can store the $k$ coefficients of the form $(2d - 1)^{j}$ such that, $0 \leq j < k$ using $O(\log\log^{t}|U|)$ space and with one-time computation complexity $O(k\log k) = O(\log\log^t|U|)$ for some constant $t$. Using these coefficients and the permutation of the digits the verifier can construct a number of that sequence in $O(k) = O(\log\log^t|U|)$ time for some constant $t$. So the total verifier time for all updates is $O(5n\log\log^tn) = O(n\log\log^tn) \text{ as } |U| \leq n$ for some constant $t$. 

\item $f_{A}(i)$ mod $5 = 2$, $\forall i \in [r]$.\\
By pigeonhole principle, there must be some $C_j$ for $j \in [5]$ such that $\left| C_j \right| \geq r$. The verifier can keep $5$ counters, one for each of the modulo classes, and can keep incrementing as it generates $5r$ numbers in the previous step. Finally it will remember the $j$ for which $\left| C_j \right| \geq r$. Next, verifier can get all the vertices in each connected component in a sequence and the components in the order of their ids. So verifier receives components in the following order $U_1, U_2, \ldots U_r$ and sees all the vertices in any component $U_i$, before it gets the next component. Now the verifier can simply regenerate the sequence as in previous step but this time only chooses $x \mid f_A(x) \text{ mod } 5 = j$, and it selects a new $x$ only when it receives a new component. WLOG it can be said that verifier picks a set $\{x_1, x_2, x_3, \ldots x_r\}$ corresponding to $\{U_1, U_2, \ldots U_r\}$. And finally it chooses $f_A(x) = f_A(x) + 2 - j$ where $x \in [1\ldots r]$ to ensure the sequence is $2 \mod 5$ while still possessing $3$-AP free property. So this step also takes $O(n\log\log^tn)$ verifier time for all updates as shown before.

\end{itemize}


==> mwmg.tex <==
\section{SIP for Maximum-Weight-Matching in General Graphs}
\label{sec:mwmg}

We now turn to the most general setting: of maximum weight matching in general graphs and the bipartite case is presented in Appendix \ref{sec:maxWBipartite}. This of course subsumes the easier case of maximum cardinality matching in general graphs, and while there is a slightly simpler protocol for that problem based on the Tutte-Berge characterization of maximum cardinality matchings \cite{tutte,berge}, we will not discuss it here. 

%Our verification protocol will introduce another technique we call ``flattening''. 

We will use the odd-set based LP-duality characterization of maximum weight matchings due to Cunningham and Marsh. 
Let $\mathbb{O}(V)$ denote the set of all odd-cardinality subsets of $V$
Let $y_i \in [n^c]$ define non-negative integral weight on vertex $v_i$,   $z_U \in [n^c]$ define a non-negative integral weight on an \emph{odd-cardinality} subset $U \in \mathbb{O}(V)$,  $w_{ij} \in [n^c]$ define the weight of an edge $e = (i,j)$ and $c^* \in [n^{c+1}]$ be the weight of a maximum weight matching on $G$. 
We define $y$ and $z$ to be \emph{dual feasible} if $y_i+ y_j + \sum_{\substack{ U \in \odd(V)  \\ i,j \in  U }   } z_U \geq w_{i,j}, \forall i,j $

A collection of sets is said to be \emph{laminar} if any two sets in the collection are either disjoint or nested (one is contained in the other). Note that such a family must have size linear in the size of the ground set. Standard LP-duality and the Cunningham-Marsh theorem state that:

\begin{theorem}[\cite{cm}]
\label{thm:cm}
For every integral set of edge weights $W$, and choices of dual feasible integral vectors $y$ and $z$,
$c^* \leq \sum_{v\in V} y_v +\sum_{U \in \odd(V)} z_U  \left \lfloor \frac{1}{2} |U| \right \rfloor.$
Furthermore, there exist vectors $y$ and $z$ that are dual feasible such that $\{ U : z_U > 0 \}$ is laminar and for which  the above upper bound achieves equality.
\end{theorem}

% Theorem~\ref{thm:cm} tells us that \textsf{P} can provide a certificate of size $O(|V|)$: the $n$ $y_i$ values as well as all non-zero $z_U$, which must be linear in number by virtue of forming a laminar family. 

We design a protocol that will verify that each dual edge constraint is satisfied by the dual variables. The laminar family $\{ U : z_U > 0 \}$ can be viewed as a collection of nested subsets (each of which we call a \emph{claw}) that are disjoint from each other. Within each claw, a set $U$ can be described by giving each vertex $v$ in order of increasing \emph{level} $\ell(v)$: the number of sets $v$ is contained in (see Figure \ref{fig:laminar})
\begin{figure}[h!]
  \centering
%    \includegraphics[width=0.5\textwidth]{lamExample}
\includegraphics[width=0.5\textwidth]{laminar}
  \caption{A Laminar family\label{fig:laminar}}

\end{figure}
The prover will describe a set $U$ and its associated $z_U$ by the tuple $(LI, \ell, r_U, \partial U)$, where $1 \leq LI \leq n$ is the index of the claw $U$ is contained in, $\ell = \ell(U)$, $r_U = \sum_{U' \supseteq U'} z_{U'}$ and $\partial U = U \setminus \cup_{U'' \subset U} U''$. For an edge $e = (i,j)$ let $r_e = \sum_{i,j \in U, U \in \odd(V)} z_U$ represent the weight assigned to an edge by weight vector $z$ on the laminar family. Any edge whose endpoints lie in different claws will have $r_e = 0$. For a vertex $v$, let $r_v  = \min_{v \in U} r_U$. For an edge $e = (v,w)$ whose endpoints lie in the same claw, it is easy to see that $r_e = \min(r_v, r_w)$, or equivalently that $r_e = r_{\arg \min (\ell(v), \ell(w))}$. For such an edge, let  $\ell_{e, \downarrow} = \min (\ell(u), \ell(v))$ and $\ell_{e, \uparrow} = \max (\ell(u), \ell(v))$. We will use $LI(e) \in [n]$ to denote the index of the claw that the endpoints of $e$ belong to. 
\vspace*{-3mm}
\paragraph*{The Protocol.}
\vspace*{-2mm}
\textsf{V} prepares to make updates to a vector $\mathbf{a}$ with entries indexed by $\mathcal{U} = \mathcal{U}_1 \cup \mathcal{U}_2$.  $\mathcal{U}_1$ consists of all tuples of the form $ \{ (i,j, w, y, y', LI, \ell, \ell', r)\}$ and $\mathcal{U}_2$ consists of all tuples of the form $ \{ (i,j,w, y, y',0,0,0,0) \}$
 where $i < j, i, j, LI, \ell, \ell' \in [n]$, $y, y',r, w \in [n^c]$ and tuples in $\mathcal{U}_1$ must satisfy  1) $w \leq y + y' + r$ and 2) it is \emph{not} simultaneously true that $y + y' \geq w$ and $r > 0$. Note that  $\mathbf{a} \in \integers^u$ where $u = O(n^{4c + 5})$ and all weights are bounded by $n^c$. 
\begin{enumerate}
\item \textsf{V} prepares to process the stream for an $F^{-1}_5$ query. When $\textsf{V}$ sees an edge update of form $(e, w_e, \Delta)$, it updates all entries  $\mathbf{a}[(e, w_e, *, *, *, *, *, *)]$. 
\item \textsf{P} sends a list of vertices $(i, y_i)$ in order of increasing $i$. For each $(i, y_i)$, \textsf{V} increments by $1$ the count of all entries $\mathbf{a}[(i, *, *, y_i, *, *, * , * , *]$ and  $\mathbf{a}[(*,i,*, *, y_i, *,*, *,*)]$ with indices drawn from $\mathcal{U}_1$. Note that \textsf{P} only sends vertices with nonzero weight, but since they are sent in increasing order, \textsf{V} can infer the missing entries and issue updates to $\mathbf{a}$ as above. \textsf{V} also maintains the sum of all $y_i$. 
\item \textsf{P} sends the description of the laminar family in the form of tuples $(LI, \ell, r_U, \partial U)$, sorted in lexicographic order by $LI$ and then by $\ell$. \textsf{V} performs the following operations.
  \begin{enumerate}
  \item \textsf{V} increments all entries of the form $(i, *,*, y_i, *, 0, 0 , 0 , 0)$ or $(*,i,*, *, y_i, 0,0, 0,0)$ by $2$ to account for edges which are satisfied by only vector $y$.
  \item \textsf{V} maintains the sum $\Sigma_R$ of all $r_U$ seen thus far. If the tuple is deepest level for a given claw (easily verified by retaining a one-tuple lookahead) then \textsf{V} adds $r_U$ to another running sum $\Sigma_{\max}$. 
  \item \textsf{V} verifies that the entries appear in sorted order and that $r_U$ is monotone increasing. 
  \item \textsf{V} updates the fingerprint structure from Theorem \ref{thm:multi-set-equality} with each vertex in $\partial U$. 
  \item  For each $v \in \partial U$, \textsf{V} increments (subject to our two constraints on the universe) all entries of $\mathbf{a}$ indexed by tuples of the form $(e, w_e, *, *, LI, *, \ell, *)$ and all entries indexed by tuples of the form $(e, w_e, *, *, LI, \ell, *, r_U)$, where $e$ is any edge containing $v$ as an endpoint. 
\item \textsf{V} ensures all sets presented are odd by verifying that for each $LI$, all $|\partial U|$ except the last one are even. 
  \end{enumerate}
\item \textsf{P} sends \textsf{V} all vertices participating in the laminar family in ascending order of vertex label. \textsf{V} verifies that the fingerprint constructed from this stream matches the fingerprint constructed earlier, and hence that all the claws are disjoint. 
\item \textsf{V} runs a verification protocol for $F^{-1}_5(\mathbf{a})$ and accepts if $F^{-1}_5(\mathbf{a}) = m$, returning $\Sigma_r$ and $\Sigma_{\max}$.
\end{enumerate}

Define $c^s$ as the certificate size, which is upper bounded by the matching cardinality. Then:
\begin{theorem}
  Given dynamic updates to a weighted graph on $n$ vertices with all weights bounded polynomially in $n$, there is a SIP with cost $(\log^2 n, (c^s + \log n) \log n)$, where $c^s$ is the cardinality of maximum matching, that runs in $\log n$ rounds and verifies the size of a maximum weight matching.
\end{theorem}
\begin{proof}
In parallel, \textsf{V} and \textsf{P} run protocols to verify a claimed matching as well as its optimality. The correctness and resource bounds for verifying the matching follow from Section~\ref{sec:mcmb}. We now turn to verifying the optimality of this matching. 
  The verifier must establish the following facts:
  \begin{inparaenum}[(i)]
  \item \textsf{P} provides a valid laminar family of odd sets
  \item The lower and upper bounds are equal. 
  \item All dual constraints are satisfied
  \end{inparaenum}

Since the verifier fingerprints the vertices in each claw and then asks \textsf{P} to replay all vertices that participate in the laminar structure, it can verify that no vertex is repeated and therefore that the family is indeed laminar. Each $\partial U$ in a claw can be written as the difference of two odd sets, except the deepest one (for which $\partial U = U$. Therefore, the cardinality of each $\partial U$ must be even, except for the deepest one. \textsf{V} verifies this claim, establishing that the laminar family comprises odd sets. 

Consider the term $\sum_U z_U\lfloor |U|/2 \rfloor$ in the dual cost. Since each $U$ is odd, this can be rewritten as $(1/2)( \sum_u z_u |U| - \sum_U z_U)$. Consider the odd sets $U_0 \supset U_1 \supset \ldots \supset U_l$ in a single claw. We have $r_{U_j} = \sum_{i \le j} z_{U_i}$, and therefore $\sum_j r_{U_j} = \sum_j \sum_{i\le j} z_{U_i}$. Reordering, this is equal to $\sum_{i \le j} \sum_j z_{U_i} = \sum_i z_{U_i} |U_i|$. Also, $r_{U_l} = \sum_i z_{U_i}$. Summing over all claws, $\Sigma_r = \sum_U z_U |U|$ and $\Sigma_{\max} = \sum_U z_U$. Therefore, $\sum_i y_i + \Sigma_r - \Sigma_{\max}$ equals the cost of the dual solution provided by \textsf{P}. 


Finally we turn to validating the dual constraints. Consider an edge $e = (i,j)$ whose dual constraints are satisfied: i.e \textsf{P} provides $y_i, y_j$ and $z_U$ such that $y_i + y_j + r_{ij} \ge w_e$. Firstly, consider the case when $r_{ij} > 0$. In this case, the edge belong to some claw $LI$. Let its lower and upper endpoints vertex levels be $s, t$, corresponding to odd sets $U_S, U_t$. Consider now the entry of $\mathbf{a}$ indexed by $(e, y_i, y_j, LI, s, t, r_{ij})$.  This entry is updated when $e$ is initially encountered and ends up with a net count of $1$ at the end of input processing. It is incremented twice when \textsf{P} sends the $(i, y_i)$ and $(j, y_j)$. When \textsf{P} sends $U_s$ this entry is incremented because $r_{ij} = r_{U_s} = \min (r_{U_S}, r_{U_t})$ and when \textsf{P} sends $U_t$ this entry is incremented because $U_t$ has level $t$, returning a final count of $5$. If $r_{ij} = 0$ (for example when the edge crosses a claw), then the entry indexed by $(e, w_e, y_i, y_j, 0,0,0,0)$ is incremented when $e$ is read. It is not updated when \textsf{P} sends $(i, y_i)$ or $(j, y_j)$. When \textsf{P} sends the laminar family, \textsf{V} increments this entry by $2$ twice (one for each of $i$ and $j$) because we know that $y_i + y_j \ge w_e$.  In this case, the entry indexed by $(i,j,w_e,y_i,y_j,0,0,0,0)$ will be exactly $5$. Thus, for each satisfied edge there is exactly one entry of $\mathbf{a}$ that has a count of $5$.

Conversely, suppose $e$ is not satisfied by the dual constraints, for which a necessary condition is that $y_i + y_j < w_e$. Firstly, note that any entry indexed by $(i,j,w_e, *, *, 0,0,0,0)$ will receive only two increments: one from reading the edge, and another from one of $y_i$ and $y_j$ but not both. Secondly, consider any entry with an index of the form $(i,j,w_e, *, *, LI, *, *, *)$ for $LI > 0$. Each such entry gets a single increment from reading $e$ and two increments when \textsf{P} sends $(i, y_i)$ and $(j, y_j)$. However, it will not receive an increment from the second of the two updates in Step 3(e), because $y_i + y_j + r_{ij} < w_e$ and so its final count will be at most $4$. The complexity of the protocol follows from the complexity for \finv, \subgraph and the matching verification described in Section \ref{sec:mcmb}. 
\end{proof}

% \paragraph{Flattening}

% A key trick we use here is to use a separate entry of $\mathbf{a}$ for each \emph{value} of an edge weight or dual variable. The key is to observe that the communication cost of our protocols depends linearly on the maximum value of an element of $\mathbf{a}$, but only \emph{logarithmically} on the length of the vector itself. So if we can ``flatten'' the vector so that it becomes larger, but the maximum value of an element becomes smaller, we might obtain a cheaper protocol. 

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "verify_matchings"
%%% End:

